AI Greenferencing: Routing AI Inferencing to Green Modular Data Centers with Heron

AI power demand is growing unprecedentedly thanks to the high power density of AI compute and the emerging inferencing workload. On the supply side, abundant wind power is waiting for grid access in interconnection queues. In this light, this paper argues bringing AI workload to modular compute clusters co-located in wind farms. Our deployment right-sizing strategy makes it economically viable to deploy more than 6 million high-end GPUs today that could consume cheap, green power at its source. We built Heron, a cross-site software router, that could efficiently leverage the complementarity of power generation across wind farms by routing AI inferencing workload around power drops. Using 1-week ofcoding and conversation production traces from Azure and (real) variable wind power traces, we show how Heron improves aggregate goodput of AI compute by up to 80% compared to the state-of-the-art.

==> design.tex <==

\section{\rname design}
\label{sec:Design}

\lccomment{IMO, one of the biggest risks of this paper being rejected is the possibility that a negative reviewer might perceive it as `yet another ILP solver' with limited solution novelty.
To address this:
\begin{itemize}
    \item 
    Consider making 3.1 a standalone section to clearly highlight what is unique/challenging about the design space considerations of \rname over a naive cross-site router people may have in mind (in fact, the section can start with picturing this strawman solution and then dive into what's wrong with it!).
    The current 3.1 seems to aim for this, but it undersells the problem and loses the audience IMO.
    Some of the root causes:
    \begin{itemize}
        \item Irrelevant content: Avoid mixing in opportunities or \rname-specific ideas, which would fit better in later design sections.
        \item Ad-hoc presentation: The current list of arguments appears scattered, and it took some time for a reader to form a coherent view. 
    \end{itemize}
    
    \item Similar issues apply to Section 3.2.
    Elevate it to a standalone section as well and use subsections for each component (e.g., Planner-L). 
    Within each component, tell a story with clarity on the rationale behind each sub-goals and design decisions, assuming that a reader will ignore the ILP equations (at least for the first evaluation pass).
\end{itemize}
As a style reference, I recommend looking at Sections 3 and 4 of the classic SWAN paper (\cite{hong2013achieving}), which precisely capture what I had in mind.
}

\subsection{System design challenges}
\label{subsec:sys_design_challenges}
Running AI inferencing workload in wind farms is challen\-ging---alongside all the feasibility and economic concerns that we addressed above, we also need to explore multiple non-trivial system design challenges. 
It is important to quantify the nuances of the workload, anticipate the residual (after deploying compute at a lower percentile of generation) power variability per site, and then match the temporally changing workload demand with the changing power (and hence compute) availability, still catering to the different latency SLOs. Below we briefly touch upon each of the system design challenges that assist us in understanding better the AI Greenferencing design choices made.

\parab{Workload characteristics.} In this work we focus on large language model (LLM) inferencing---it is unique in terms of diverse mix of user requests and responses and the rich availability of both application and hardware knobs that could be leveraged for right-sizing the power consumption. Different LLM models (with different context lengths) could have diverse input and output lengths, and latency SLOs, and could be run with different tensor parallelism (TP) and frequency capping configurations. We ran a deep power profiling benchmark, as we discuss in \S\ref{sec:results}, building on top of past work~\cite{dynamollm} but for more recent Llama $3.1$ $70$~B model. We classify inferencing requests based on their input and output lengths, quantify plausible latency SLOs, and quantify how different degrees of TP and frequencies could run the same request class (at different levels of load or requests per second) at different power and latencies. The profiling exercise helps us obtain $2$ useful functions -- $1$. \textit{e$2$e($c$, $f$, $t$, $l$)} that gives the end-to-end latency and $2$. \textit{power($c$, $f$, $t$, $l$)} that gives the peak power consumed by the $c$-th class of requests at load $l$ run with TP $t$ and GPU frequency $f$. In a dynamic setting with total available power being lower at times than the peak demand, it is important to leverage these tuning knobs well to remain within the resource constraints but still cater to the workload. The state-of-the-art DynamoLLM scheduler~\cite{dynamollm} (our baseline; discussed further in \S\ref{sec:related_work}) that aims to minimize power/energy consumption, assumes infinite hardware and power availability in a traditional data center. AI Greenferencing rather is deployed on modular data centers in wind farms and is, hence, constrained by power and hardware. We discuss the profiling results in \S\ref{subsec:results:profiling}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/SLO_Violations.png}
    %\vspace{-0.35in}
    \caption{DynamoLLM needs to drop requests in the absence of cross-site intelligence that could leverage power generation complementarity.}
    %\vspace{-12pt}
    \label{fig:dynamo:slo}
\end{figure}
\parab{Temporal variations in demand and supply.} Both AI inferencing workload arrival rate (demand) and power generated at individual wind farm sites could vary over time. AI Greenferencing absorbs these temporal variations by leveraging spatial complementarity, as touched upon in \S\ref{sec:feasibility}. While the deployed AI compute receives peak power most of the time, thanks to right-sizing the provisioned hardware (see \S\ref{sec:provisioning}), the residual variations across wind farms often do not coincide, leading to cross-site software routing opportunities. Fig.~\ref{fig:dynamo:slo} demonstrates this opportunity. The AI Inferencing workload (real trace) is sent across $2$ wind farm sites in the UK (compute provisioned for peak demand of $13.25$~MW) and Iceland (likewise, $29$~MW). Each site runs a DynamoLLM scheduler that minimizes the energy consumption. We see that at times between $285$-$315$~min for the Iceland site and $435$-$630$, $1$,$320$-$1$,$395$, $1$, and $470$-$1$,$755$~min for the UK site, the available power drops below the provisioned power and also the minimum energy ask of the assigned workload thus resulting in significant request drops (bottom plot, normalized by the peak). \textit{All} these drops could have been avoided by routing around `bad' power conditions as the combination of the sites offered full complementarity during this time window.

\parab{Compute cluster reconfigurations.} As discussed above, AI Greenferencing scheduler could leverage ($1$) knobs such as TP and frequency capping across clusters of GPUs and ($2$) cross-site routing to deal with workload arrival and power generation uncertainties. Changing GPU frequencies take milliseconds via \texttt{nvidia-smi} and changing TP take a few seconds to minutes due to the multiple steps involved -- waiting for existing requests to complete, re-sharding the model weights, transferring them to the GPUs involved, and synchronizing the GPUs. \rname minimizes the number of TP and frequency reconfigurations. The complementarity of generation across sources results in spatial redundancy/diversity of generation aiding \rname's strategy further. \rname also adopts DynamoLLM~\cite{dynamollm} optimizations (using inter-GPU NVLink and transferring weights between GPUs in the background) toward minimizing re-sharding overheads during TP reconfigurations.

\parab{Handling mispredictions.} Wind power generation could be predicted with high accuracy at $15$~min granularity, as discussed in \S\ref{sec:feasibility}. \rname uses these predictions to plan ahead the workload routing across multiple sites. Nevertheless, there could be inaccuracies in both workload arrival and power generation predictions that are needed to be handled online. To address this, we resort to hierarchical decision making (different temporal granularity) as we discuss next.

\greybox{We need a cross-site router that is power variability aware, workload variability \& characteristics aware, and could effectively leverage the power complementarity across sites, and the application (TP) and infrastructural (GPU frequency) knobs.}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/system/system_design.png}
    %\vspace{-0.35in}
    \caption{AI Greenferencing architecture.}
    %\vspace{-12pt}
    \label{fig:architecture}
\end{figure}

\subsection{\rname components}
\rname consists of multiple components as seen in Fig.~\ref{fig:architecture}. The goal of \rname is to determine number of GPUs, TP degree, frequency and load for each request class at each renewable site. While changing TP degree could take few seconds to minutes due to (potential) resharding of model weights, frequency and load can be changed within milliseconds. To take into account these different timescales, we decompose \rname into three key components that run at different timescales: \texttt{Planner-L}, \texttt{Planner-S}, and \texttt{Request Scheduler with a packing heuristic}. \texttt{Planner-L} runs at a coarser timescale (e.g., $15$~min) and assigns the TP degree, frequency, and load. However, such coarser timescale assignments are less reactive to real-time power and workload conditions. We built \texttt{Planner-S} that considers changing conditions at finer timescales and updates the frequency and load (these changes can be done quickly) while sticking to the TP assignments done by Planner-L. We also built a real-time \texttt{packing heuristic} that runs alongside the \texttt{Request Scheduler} to further handle the changing conditions and unleash performance. We detail these components below.

%\rohan{The goal of \rname is to determine number of GPUs, TP degree, frequency and load for each request class at each renewable site. Note that changing TP degree at GPUs is a time consuming operation and requires (potentially) resharding model weights. Such operations can take minutes and could be disruptive to existing requests. In contrast, frequency and load can be changed quickly. To take into account different timescales, we decompose \rname across three components that run at different timescales: Planner-L, Planner-S and a heuristics. Planner-L assigns the TP degree, frequency and load and runs at coarser timescales as: (a) changing TP degrees take time. (b) power and workload predictions are available at minutes granularity. However, such coarser timescale assignments do not react to real time power and workload conditions. We built Planner-S that considers near real-time conditions and updates the frequency and load (these changes can be done quickly) while sticking to the TP assignments done by Planner-L. We also built heuristics to further handle the real-time conditions. We details these components next. }

\input{planner_L}
\parab{Planner-L.} Both workload arrival and wind power generation per site are highly predictable at $15$~min granularity (see \S\ref{sec:feasibility}) and these predictions, alongside inferencing profiled data (a lookup table), are leveraged by a long-term ($15$~min) lookahead \texttt{Planner-L} ILP (integer linear program). Based on the predictions (treated as oracle), \texttt{Planner-L} comes up with a plan to configure the TP and operating frequencies of sets (instances) of GPUs per site that would then be mapped to classes (based on input and output length) of inferencing requests for the next $15$~min window. While a naive planner could lead to frequent reconfigurations of GPU clusters as power per site and workload arrival rate varies across $15$~min slots, \texttt{Planner-L} bounds such reconfigurations to further aid the DynamoLLM strategies for hiding reconfiguration overhead (that we have adopted). \texttt{Planner-L} outputs TP and frequency reconfigurations needed, and also the fraction of inferencing requests per class that should be routed to individual instances across the multiple sites. Table.~\ref{tab:algo1:notation} and Fig.~\ref{fig:plannerl:formulation} detail the notation and formulation of the ILP -- it takes as input the workload classes, TP degrees, GPU operating frequencies, load levels (requests/s) per class per instance, number of GPUs and power available per site in the next time slot, the peak load per class of requests, and previous configuration, and gives as output the optimal next configuration that minimizes end-to-end latency of inferencing. The ILP minimizes the aggregate end-to-end latency for the workload (thus not compromising on the user experience) making sure that the configuration respects the ($1$) hardware and ($2$) power availability constraints per site, ($3$) each class of requests get enough serving capacity that could satisfy the peak load, ($4$) each class of requests get the same frequency assigned for the same load, and ($6$, $7$) the number of reconfigurations needed per time slot is bounded.

\parab{Configurator.} The \texttt{Configurator} is in charge of updating the site-specific configurators of the necessary changes in TP and operating frequencies of different clusters of GPUs. While such reconfigurations are in progress, the \texttt{Configurator} restrains \texttt{Planner-S} from considering those clusters for workload placement.

\input{planner_S}
\parab{Planner-S.} While \texttt{Planner-L} runs every $15$~min and reconfigures TP, operating frequency, and load per GPU instance, we could also run a lightweight \texttt{Planner-S} that runs every few seconds to tens of seconds and reconfigures only the frequencies and the load assigned per instance, as TP changes are heavier. Running \texttt{Planner-S} at finer timescales has $2$ major benefits -- ($1$) it could tackle residual power and workload arrival uncertainties and ($2$) it could unleash performance opportunity by running requests at higher than \texttt{Planner-L} assigned GPU frequencies as the available power goes up thus improving TTFT and TBT latencies.
%While \texttt{Planner-L} runs every $15$~min and matches workload arrival rate to available power across sites, there could be deviations online. Although we see that both demand (workload) and supply (power) are highly predictable at this timescale (see \S\ref{sec:feasibility}), we need to address corner cases where they deviate from predictions due to unforeseen reasons. This also unleashes performance opportunity -- if available power goes up, requests could be run at higher than assigned GPU frequencies thus improving TTFT and TBT latencies. 
\texttt{Planner-S} is also an ILP (notations in Table.~\ref{tab:algo1:notation} and ILP in Fig.~\ref{fig:algo2:router}) that runs at a configurable cadence (more frequently than \texttt{Planner-L}) to find out the optimal frequency configurations and load assignments for GPU clusters across the sites given the current conditions. Note that \texttt{Planner-S} has the same optimization goal as \texttt{Planner-L} but only minimally reconfigures frequencies (orders of magnitude faster to do) and not the TP. \texttt{Planner-S}, like \texttt{Planner-L}, also minimizes the end-to-end latency of inferencing (both planner should work in tandem and have the same optimization objectives). The ILP variable $Z_{c,f,t,s,l}$ indicates number of instances assigned for each config (tuple of site, class and TP degree) and frequency and load. Note, only frequency and load are reassigned for individual configs. The constraints are: ($1$) power constraints are met, ($2$) the serving capacity is enough for the peak load, ($3$) fits in the same GPU budget assigned by Planner-L.

Note that both \texttt{Planner-L} and \texttt{Planner-S} formulations could be trivially changed to minimize power consumption instead of E$2$E latency.

\parab{Request Scheduler.} This component is in charge of dispatching the inference requests, as they arrive in the arrival queue, across multiple sites. It consumes the output of \texttt{Planner-S} to learn the weights with which it performs a weighted round-robin (WRR) routing for each class (input/output length) of requests across clusters of GPUs assigned to individual classes across sites. To assign classes to requests, it uses a \texttt{Request Class Predictor} that takes as inputs the request and the model, predicts the output length and, hence, the class. Our predictor consists of an Albert/DistilBert/Longformer~\cite{lan2020albertlitebertselfsupervised, sanh2020distilbertdistilledversionbert, beltagy2020longformer} layer for input embeddings followed by a regressor, and could predict the output length bucket (small/medium/long) with an accuracy of $99.95\%+$ (predicting buckets is easier than predicting absolute output lengths). Hence, following the footsteps of DynamoLLM~\cite{dynamollm}, we treat output length as an oracle in our experiments. The \texttt{Request Scheduler} also adds a useful \texttt{packing heuristic} -- if the observed load (requests per second) for a request class is lower than anticipated, it can move a fraction of the smaller requests to this class for better packing and performance.

\parab{Meta choices.} \rname could be deployed either at the ingress of the AI provider network or close to a full-fledged data center such that it could intercept the workload arrival. We have deliberately excluded a full-fledged data center and battery/generator capacity per site to stress test \rname's robustness in tackling the residual (post right-sizing the compute deployment) uncertainties in power and workload arrival. \rname could essentially work with any wind site-local scheduler, but in this work we have first-in-first-out round-robin (in GPU assignment) schedulers per site.



==> eval.tex <==
\section{Evaluation}
\label{sec:eval}

\subsection{Performance of Planner-L}
\label{sec:eval:plannerl}

\if 0
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth, page=1]{eval-figs/eval-summary.pdf}
    %\vspace{-0.35in}
    \caption{Latency and Power in Planner-L and other methods.}
    \label{fig:eval:summary}
\end{figure}
\fi

%%%%%%%%%% figure start %%%%%%%%%%%%%%%%
\begin{figure}[tbh]
\centering
\subfigure[Latency]
{
\includegraphics[width = 0.45\textwidth, page=1]{eval-figs/eval-summary.pdf}
\label{fig:eval:summary:lat}
}
\\
\subfigure[Power]
{
\includegraphics[width = 0.45\textwidth, page=2]{eval-figs/eval-summary.pdf}
\label{fig:eval:summary:pow}
}
\caption{Latency and power across different methods.}
\protect\label{fig:eval:summary}
\end{figure}
%%%%%%%%%%%%%%%%%%%%% figure end %%%%%%%



%%%%%%%%%% figure start %%%%%%%%%%%%%%%%
\begin{figure}[tbh]
\centering
\subfigure[Latency]
{
\includegraphics[width = 0.45\textwidth, page=3]{eval-figs/eval-summary.pdf}
\label{fig:eval:summary:lat}
}
\\
\subfigure[Power]
{
\includegraphics[width = 0.45\textwidth, page=4]{eval-figs/eval-summary.pdf}
\label{fig:eval:summary:pow}
}
\caption{Timeseries of latency and power consumed in 1 week.}
\protect\label{fig:eval:timeseries}
\end{figure}
%%%%%%%%%%%%%%%%%%%%% figure end %%%%%%%

Fig.\ref{fig:eval:summary} shows the latency and power consumed by all the 5 methods. We run all methods every 15 mins for a 7 day period. We report the average latency and power. We make the following observations: (a) Planner-L-min-latency achieves the lower end-to-end (e2e) latency using an ILP. Compared to baseline-latency that also tries to lower e2e latency, Planner-L-min-latency results in XX\% lower latency. However, Planner-L-min-latency also results in the highest power consumed. Note that, Planner-L-min-latency never exceeds the available power at individual sites. 

In contrast, we also compare the methods that optimize for power. Compared to DynamoLLM, Planner-L-min-power results in lower latency and power up to 15\%. Further, Planner-L-dynpower that consumes the same power as DynamoLLM results in lower latency of 25\% for LLama3 workloads. For LLama2 workload, we observed up to 74\% improvement in e2e latency. The benefits are stemming from \rohan{complete this.}

Fig.\ref{fig:eval:timeseries} shows the timeseries of latency and power for the 7-day period for Llama3-coding. It can be seen that Planner-L-min-latency consistently achieves lower latency than other methods. Similarly, compared to DynamoLLM, Planner-L-dynpower achieves lower latency.

\subsection{Impact of different traffic rates}
\label{sec:eval:traffic}


%%%%%%%%%% figure start %%%%%%%%%%%%%%%%
\begin{figure}[tbh]
\centering
\subfigure[Latency]
{
\includegraphics[width = 0.45\textwidth, page=5]{eval-figs/eval-summary.pdf}
\label{fig:eval:summary:lat}
}
\\
\subfigure[Power]
{
\includegraphics[width = 0.45\textwidth, page=6]{eval-figs/eval-summary.pdf}
\label{fig:eval:summary:pow}
}
\caption{Latency and power when varying traffic.}
\protect\label{fig:eval:traffic}
\end{figure}
%%%%%%%%%%%%%%%%%%%%% figure end %%%%%%%

In this section, we use LLama3-coding workload and vary the request rates. We label unchanged request rate as 100\% and we vary the request rate to 80\% and 120\%. Fig.\ref{fig:eval:traffic} shows the latency and power across 5 methods from previous section.

It can be seen that the latency increase is very minimal even at 120\% traffic. This is primarily because of two factors: (a) there are enough GPUs to handle surge in the traffic, (b) we did observe higher load on GPUs in events number of GPUs is saturated. However, due to the intrinsic nature of the latency vs. load curve, the latency increase is minimal. Note that the latency vs. load curve observes knee points, where  the latency increase is minimal while increase load (up to a certain load point). 

\subsection{Impact of reconfiguration}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth, page=7]{eval-figs/eval-summary.pdf}
    %\vspace{-0.35in}
    \caption{Impact of reconfiguration limit on latency and power.}
    \label{fig:eval:reconf}
\end{figure}

In this section, we evaluate Planner-L where we set a limit of possible reconfigurations ($R_{L}$ in Fig.\ref{fig:plannerl:formulation}. We consider $R_{L}$ as 10\%, 5\%, 2\% and 0.5\% of total number of GPUs. We compare the latency and power against a baseline where we do not have any limit. As shown in Fig.\ref{}, even when the $R_{L}$ is as low as 2\%, there is roughly no change in latency and power. This is because the power and loads (RPS) do not change suddenly -- the changes are more gradual. Consequently, Planner-L is able to pack the requests even with $R_L$ of 2\%. However, for the $R_L$ of 0.5\%, we see an increase in e2e latency. Such an $R_L$ is not enough to pack the requests, and Planner-L ends up making suboptimal decisions (compared to having no reconfiguration limit).    

\subsection{Planner-L scalability}

\subsection{Heuristic}
\subsubsection{Algorithm to minimize e2e latency description}
\raja{
We are given the provisioning of the maximum load (Requests per Second, RPS) for each class for the next 5 seconds, and there are 9 classes in total. The key points of the algorithm are:
\begin{itemize}
    \item A class $X$ can run on a class $Y$'s configuration without SLO violations if both the input and output of $Y$ are greater than or equal to $X$'s input and output classes. For example, ML can only run on LL but not on LM or LS.
    \item We calculate the e2e latency benefit of transitioning a request from class $X$'s configuration to all permitted class $Y$ configurations for all classes and store these data in a lookup table (LUT).
    \item Every second, we iterate through the incoming loads from the LL class to the SS class: \begin{itemize}
        \item If the incoming load for a class is less than its provisioned load, we use the LUT and shift the load from other classes based on the benefit value in descending order.
    \end{itemize}
\end{itemize}
}
% \begin{table}[]
% \caption{Permitted Transitions}
% \label{tab:heuristic:1}
% {
% \small
% \begin{tabular}{|p{0.27\columnwidth}|p{0.65\columnwidth}|}
% \hline
% \textbf{Class X} & \textbf{Class Y} \\ \hline
% LM & LL \\ \hline
% LS & LM, LL \\ \hline
% ML & LL \\ \hline
% MM & ML, LM, LL \\ \hline
% MS & MM, ML, LS, LM, LL \\ \hline
% SL & ML \\ \hline
% SM & SL, MM, ML, LM, LL \\ \hline
% SS & SM, SL, MS, MM, ML, LS, LM, LL \\ \hline
% \end{tabular}
% }
% \end{table}
% \subsubsection{Pseudocode}

\begin{algorithm}
\caption{Load Transition Based on Benefit Values}
\label{alg:load_transition}
\begin{algorithmic}[1]
\STATE \textbf{Input:}
\STATE Provisioned\_load[class] $\gets$ Provisioned max RPS for each class (for next 5 seconds)
\STATE Incoming\_load[class] $\gets$ Incoming RPS for each class (updated every second)
\STATE LUT[class] $\gets$ Look-Up Table with benefits: \{class $X \to$ class $Y$ $\to$ benefit\}

\STATE \textbf{Initialization:}
\STATE Current\_config[class] $\gets$ Initial configuration for each class

% \WHILE{true} 
\COMMENT{Repeat every second for 5 seconds}
\STATE Update Incoming\_load[class] for all classes
    \FORALL{class in classes (sorted from LL to SS)}
    \IF{Incoming\_load[class] $<$ Provisioned\_load[class]}
        \STATE Fetch possible transitions and associated benefits from LUT[class]
        \STATE Sort other classes based on benefit values in descending order
        \FORALL{sorted classes based on benefit values}
            \STATE Shift load from current\_config[class] to new configuration based on maximum benefit
        \ENDFOR
    \ENDIF
\ENDFOR
% \ENDWHILE
\end{algorithmic}
\end{algorithm}

% \begin{table}[]
% \caption{Priority Order}
% \label{tab:heuristic:2}
% {
% \small
% \begin{tabular}{|p{0.27\columnwidth}|p{0.65\columnwidth}|}
% \hline
% \textbf{Parent class} & \textbf{Child class} \\ \hline
% LL & LM, ML, LS, SL, MM, MS, SM, SS \\ \hline
% LM & LS, MM, MS, SM, SS \\ \hline
% LS & MS, SS \\ \hline
% ML & MM, SL, MS, SM, SS \\ \hline
% MM & MS, SM, SS \\ \hline
% MS & SS \\ \hline
% SL & SM, SS \\ \hline
% SM & SS \\ \hline
% \end{tabular}
% }
% \end{table}

\subsubsection{Algorithm to maximize request shifting description}
\raja{
The main difference between the previous algorithm and this is the order of choosing the classes to shift when there is a vacancy in a class. Previously, the order was based on the e2e benefits, now the order is to try and move as many requests as possible. When there is a vacancy in class LL, we can pick requests from any one of the classes and move there. But if we move SS to LL, then there is a vacancy in SS and no other requests can be moved there as they would violate the SLOs. But if we move a MM request for example, the other requests from lower class can be moved here. 
% Table~\ref{tab:heuristic:2} shows the priority order of all permitted child classes for the transition to the parent class.
The priority order was made by taking into account the number of possible transitions for each child clash and giving higher priority to the larger input in case of clash between two classes. For example, both LS and SL have only 2 possible transitions LM \& LL and ML \& LL respectively. For LL as the parent class, LS will be given a higher priority over SL.
}



==> motivation.tex <==
\section{Broad idea \& motivation}
\label{sec:motivation}

==> notes.tex <==

\section{Power profiling at different granularities}
Q. Why do need the profiling data at a finer granularity, what are the benefits?\\
A. Now we have the power numbers for each class for different loads at different frequencies. This profiling is done by taking the input and output length around the threshold numbers. For example for SM we take inputs from TH(short)-10 to TH(short) and for output TH(medium)-10 to TH(medium). But in reality all the queries from input(0 - TH(short)) and output(TH(short) to TH(medium)) are considered as SM. To avoid this we will need profiling data at a finer granularity. \\
 
Q . What we can do for this? \\
A. For every class we can have 100 subclasses further, this data will be used by the Online Router and the class wise data will be used by the LP. \\
 
Q. How do we make these 100 subclasses?\\
A. To illustrate, let's consider a short input range from 0-290 and a short output range from 0-100. We can create 10 subclasses for the input (0-29, 29-58, ..., 261-290) and 10 subclasses for the output (0-10, 10-20, ..., 90-100). We then profile all possible combinations of these subclasses, resulting in 100 combinations (10*10).

\section{Why LP can give multiple configs{TP,Freq} for a class?}
\begin{itemize}
    \item The configuration of a cluster for a class depends on the load which it is taking, so there can be multiple configs by the LP for the same class.
    \item We are primarily working with two constraints: power budget and SLAs. Therefore, it is not always necessary to have a power-efficient configuration, as long as we adhere to these constraints.
\end{itemize}

\section{How load is interpreted?}
\begin{itemize}
    \item The LP runs every 15 minutes, the time period of 15 minutes is because we have the power data for 15 minutes. 

\item Q. Assume the GPU (TP-x, Freq-y) is provisioned to run at 5 RPS load, if we get a load of 5 RPS in consecutive timestamps how is this managed? //

Ans. The max RPS for a configuration is calculated using the profiling exercise. During the profiling exercise, we send the requests in a poisson arrival fashion maintaining the average RPS as load for a time period of 300s. In this method the various combinations are captured – only prefill, only decode and prefill + decode. A load is considered to be valid only if the SLOs are maintained throughout. This arrival of getting the provisioned RPS in consecutive seconds is captured in the profiling exercise. In terms of power, the prefills for a load at time t are done by the time t+1 when the new load arrives. The peak power is consumed during the prefills and less than average during the during the decode.  

\item Q. Are we holding the requests for 1 second and later sending them for inference? 
\\
Ans. No, we are not holding the requests for 1 second. We are doing things in anticipation. At t = 0 we anticipate that we will get 5 requests in the next second and provision for that. 

\item Q. At the time of scheduling a load on to a GPU, for calculating the power do we take into account of the existing requests, or do it use just the incoming requests? 
\\
Ans. To a GPU we will not be sending more than the provisioned RPS, as mentioned previously the power profiling uses the poisson arrival so many combinations are captured. So, to calculate the power we take the load as max of running load and the incoming load. 
\end{itemize}


==> planner_S.tex <==
% \if 0
% \begin{table}[]
% \caption{Notations: ILP for Planner-S}
% \label{tab:algo2:notation}
% {
% \small
% \begin{tabular}{|p{0.27\columnwidth}|p{0.65\columnwidth}|}
% \hline
% \textbf{Notation} & \textbf{Description}\\
% \hline
% %\hline
% %\multicolumn{2}{|c|}{Inputs} \\
% %\hline
% $CurrentPower_{s}$ & Current power at site $s$\\
% \hline
% $CurrentLoad_{c}$ & Current load for class $c$\\
% \hline
% $ConfLoad(s,c,t)$ & Load per instance for site $s$, class $c$, TP $t$\\
% \hline
% $ConfInst(s,c,t)$ & Current number of instances for \{$s$, $c$, $t$\}\\
% \hline
% $Z_{c,f,t,s,l}$ & (Integer) number of instances for frequency $f$ and load $l$ assigned to \{$c$, $t$, $s$\} \\
% \hline
% \end{tabular}
% }
% \end{table}
% \fi 

% \if 0
% $NP(c,f,t,l_{o}, l_{n})$ & New power consumed \\
%  & based on old ($l_{o}$) and new load ($l_{n}$)\\
% \hline
% $NI(c,s,t,f,l_{n})$ & New instance based on current \\ 
%  & instances, and old ($l_{o}$) and new load ($l_{n}$) \\
% \hline 
% %% \multicolumn{2}{|c|}{Output Variable (binary)} \\
% %%\hline
% \fi

% \parab{\texttt{Planner-S} ILP formulation.} Fig.\ref{fig:algo2:router} shows the ILP formulation for \texttt{Planner-S}. The notations are shown in Table~\ref{tab:algo1:notation}. The ILP variable $Z_{c,f,t,s,l}$ indicates number of instances assigned to class $c$, frequency $f$, TP degree $t$, site $s$, and load $l$. Note that the class, site, and TP degree remain same (calculated by \texttt{Planner-L}) -- we only change the frequency and load. The formulation ensures that \texttt{Planner-S} remains under power and compute constraints.

% \begin{figure}[tbh!]
% {\small
% \fbox{
%   \begin{minipage}{0.97\columnwidth}
%     \textbf{ILP Variable:} $Z_{c,f,t,s,l}$\\ 
%     \textbf{Objective:} Minimize \\ $\displaystyle\sum_{s \in S, c \in C, t \in T} \displaystyle\sum_{f \in F, l \in L} Z_{c,f,t,s,l}  \cdot e2e(c,f,t,l)$\\
%     \textbf{Constraints:}\\
%     (1) Power per site within limit: \\ $\forall s \in S, \displaystyle\sum_{c, f, t, l} Z_{c,f,t,s,l} \cdot power(c,f,t,l) \leq P_{s}$ \hfill\\
%     (2) Enough serving capacity for each class: \\
%     $\forall c \in C, \displaystyle\sum_{s \in S, f \in F, t \in T, l \in L} Z_{c,f,t,s,l} \cdot l \geq Load_{c}$ \hfill\\
%     (3) Limiting number of GPUs per config:
%     \\$\forall s \in S, c \in C, t \in T, \displaystyle\sum_{l \in L, f \in F} Z_{c,f,t,s,l} \leq GPU_{s,c,t} $ \hfill
%   \end{minipage}
% }
% }
% \caption{Formulation: ILP for Planner-S}
% \protect\label{fig:algo2:router}
% \end{figure}

% \if 0
% (3) One configuration of f and l: \\$\forall s \in S, c \in C, t \in T, \displaystyle\sum_{f \in F, l \in L} W_{c,f,t,s,l} \leq 1$ \hfill (c) \\
%     (4) Expressing W in terms of Z: \\$\forall s \in S, c \in C, t \in T, f \in F, l \in L, 1 \geq W_{c,f,t,s,l} \geq \frac{Z_{c,f,t,s,l}}{sum(N_S)} $ \hfill (d)

% \fi

==> provisioning.tex <==
\section{Hardware provisioning}
\label{sec:provisioning}

\db{GPUs running AI workloads are costly~\fix{\cite{gpu_cost}}. Hence, for large AI inferencing providers spending huge CAPEX (capital expenditure) on AI compute, it is obvious to ask if deploying these costly resources at wind farms with variable power availability makes sense. Given the limited life span of GPUs, lower-than-peak power at times would entail lost compute cycles and, hence, misused CAPEX. In this section, we compare OPEX against CAPEX and find out how to provision GPUs in wind farms with modular data centers so as not to compromise on the cost of ownership.}

\lccomment{Maybe start by foreshadowing the relationship with \cref{sec:feasibility}, something like:
\cref{sec:feasibility} demonstrates the (technical) feasibility of harnessing the RE farms' power capacity with co-located GPU clusters. For cloud providers, however, TCO is a crucial consideration. This section takes a step further by analyzing its economic feasibility and answer the question: \emph{Whether the idea is beneficial for TCO, and if so, when}...
}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/provisioning/cost_vs_time.jpg}
    %\vspace{-0.35in}
    \caption{Cost of power over the lifetime of an NVIDIA H$100$ GPU could be a significant fraction of its CAPEX.}
    %\vspace{-12pt}
    \label{fig:provisioning:cost_vs_time}
\end{figure}

\subsection{OPEX versus CAPEX}
\db{The total cost of ownership (TCO) of a DC is primarily driven by $4$ components~\fix{\cite{dc_cost}}: $1$. DC CAPEX (as DC depreciation), $2$ DC OPEX, $3$. Server CAPEX (as server depreciation), and $4$. Server OPEX. Modular DCs are known~\fix{\cite{mdc_cost}} to have a low cost of production due to economies of scale -- they could be mass produced. Furthermore, when deployed on otherwise unused land in a wind farm, the cost of land acquisition or rent should also be low~\fix{\cite{wind_land}} given the revenue opportunity this deployment brings to wind farms. Hence, we do not anticipate the DC CAPEX to be any higher for AI Greenferencing deployments than for traditional DCs. In addition, modular compute deployments are easier to maintain given their standard design at scale. If wind farm employees/operators are trained to perform basic DC maintenance activities~\fix{\cite{dc_maintenance}}, this could rather bring down the DC OPEX cost further than what a traditional DC incurs. Hence, here we focus more on only the server CAPEX and OPEX aspects -- the former (driven by GPU prices) is significantly higher than traditional values for AI, and the latter (driven by the cost of power) could be significantly lower with Greenferencing style deployments, as already discussed in \fix{\S\ref{}}.}

\db{Given GPU costs have largely increased in the last few years~\fix{\cite{gpu_cost}} with NVIDIA H$100$s priced at around $30K$~USD per GPU, it could be easy to believe that CAPEX should drive server deployment choices, as the cost of power is traditionally low. Here we show otherwise -- over the lifetime of a GPU, the OPEX (cost of power in our analysis) becomes a significant fraction of the TCO. Fig.~\ref{fig:provisioning:cost_vs_time} shows the CAPEX and OPEX components of an NVIDIA H$100$ GPU normalized by its publicly quoted price of $30K$~USD. A second horizontal line (CAPEX of $20K$~USD) represents a plausible lower bound of the economies of scale for bulk buyers. All other lines show the total OPEX spent in buying power in the US and in Germany anticipating peak GPU operations throughout. As we can see, in $5$ years, the OPEX in the US is $12.4\%$ ($18.6\%$) assuming $30K$~USD (likewise, $20K$~USD) CAPEX. In Germany these numbers are much higher -- $27\%$ and $40.5\%$ respectively. In special cases, when compared against a $30K$~USD CAPEX, OPEX could be as high as $35.6\%$ in the US (California), and $61\%$ in Germany ($2022$ crisis~\fix{\cite{germany_2022}}).}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/provisioning/percentile_vs_metric_US_total.jpg}
    %\vspace{-0.35in}
    \caption{}
    %\vspace{-12pt}
    \label{fig:provisioning:percentile_vs_metric_US_total}
\end{figure}

\subsection{Better C/P than in traditional DC?}
\db{As the cost of power consumption is a significant fraction of the TCO of AI compute, we argue that it could be a better choice to lose a few GPU cycles during its lifetime if the cost of power is significantly cheaper throughout. Let us see here how a GPU deployment in a wind farm could fare against one in a traditional DC in terms of capability/price~\fix{\cite{cp_metric}} (C/P = total compute cycles / dollars spent) where the denominator is the sum of CAPEX and OPEX. Fig.~\ref{fig:provisioning:percentile_vs_metric_US_total} plots C/P for a single GPU priced at $25K$~USD over time. We assume that the GPU at its peak could sustain $10^22$~flops per year. The cost of power for enterprise customers in the US is $0.085$~USD/kWh on average, with the cost in California being $0.244$~USD/kWh as of Sep'$24$ (EIA Report~\fix{\cite{}}). On the other hand, the cost of wind power at the source, as in reported PPAs~\fix{\cite{}} (power purchase agreements), is significantly lower -- $0.025$~USD/kWh in the major wind power producing regions in the US. This lower cost of power translates to significant OPEX reductions when Ai compute is deployed at the source of power, that is the wind farms.}

\db{We do not claim that we should provision for the peak power of a wind farm -- this approach would lead to lower-than-peak power often and, hence, wasted compute cycles. Our approach, rather, is to select large wind farms and deploy at the $X^{th}$ percentile of the power generation such that only $X\%$ of the time there is lower-than-peak power (we assume half the peak provisioned, on average) for the compute deployed, while $100\%$ of the time the cost of power (hence, OPEX) is significantly cheaper. As seen in Fig.~\ref{fig:provisioning:percentile_vs_metric_US_total}, such careful provisioning of compute could lead to higher C/P in just a few years than in traditional data centers. For example, if GPUs are provisioned in a wind farm at the $5^{th}$ percentile of power generation as the peak power, wind farms deployments offer comparable or better C/P than in traditional data centers in only $2$ years. At the $15^{th}$ ($20^{th}$) percentile (larger clusters), it takes only $4$ (likewise, $5$) years to yield comparable or better C/P.} %Hence, the trick here is to pick a lower percentile of wind power generation at a farm and deploy AI compute with this bound as the peak power so that the deployment could yield comparable or higher C/P than in traditional data centers within a few years even after a few lost compute cycles due to power generation uncertainty.}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/provisioning/size_percentile_vs_hardware_operating.jpg}
    %\vspace{-0.35in}
    \caption{}
    %\vspace{-12pt}
    \label{fig:provisioning:size_percentile_vs_hardware}
\end{figure}

\subsection{High deployment appetite}

\db{The trick, as discussed above, is to pick a lower percentile of wind power generation at a farm and deploy AI compute with this bound as the peak power so that the deployment could yield comparable or higher C/P than in traditional data centers within a few years even after a few lost compute cycles due to power generation uncertainty. We observed in the ELIA dataset~\fix{\cite{}} (Flanders region, Elia grid, onshore generation) that the $X^{th}$ percentile power generation has a value significantly lower than the $X\%$ of the peak capacity -- some typical percentile-to-percentage mappings are (percentile, percentage) [($5$, $1$), ($10$, $2$), ($15$, $4$), ($20$, $5$), ($25$, $7$), ($30$, $9$)]. With this in mind, if we provision for $X^{th}$ percentile of the peak power generation capacity of a farm, it translates to a fixed number of GPU clusters. For a larger farm, we will thus have more clusters and vice versa. We now evaluate how deployment at the $20^{th}$ percentile will look like globally, if we only pick the largest (in terms of peak capacity) $Y\%$ wind farms from the global wind farm dataset~\fix{\cite{}}. For this evaluation, we assume deployments will happen in multiples of NVIDIA's H$100$ SuperPODs, each hosting $1$,$016$ H$100$ GPUs and consuming $1.3$~MW peak power. As seen in Fig.~\ref{fig:provisioning:size_percentile_vs_hardware}, the aggregate number of NVIDIA SuperPODs that could be deployed at the largest $20\%$ of the operating wind farms across the globe is $6$,$636$ -- this translates to  $6.7$~million H$100$ GPUs (more than $3\times$ the H$100$ order book of NVIDIA in $2024$~\fix{\cite{}}). Given these are all large wind farms, even the $20^{th}$ percentile ($5\%$) of peak capacity in the smallest such farm is a reasonable sized deployment of $9$ SuperPODs ($9K+$ H$100$ GPUs). In general as we pick a smaller percentile of peak power for compute right-sizing, larger the aggregate deployment but smaller the minimum deployment size (more fragmentation). This is a knob that AI inferencing providers should use based on factors like software router scalability, per-site maintenance overhead, physical security concerns, etc.}
